Minimax testing and quadratic functional estimation for circular convolution

In a circular convolution model, we aim to infer on the density of a circular random variable using observations contaminated by an additive measurement error. We highlight the interplay of the two problems: optimal testing and quadratic functional estimation. Under general regularity assumptions, we determine an upper bound for the minimax risk of estimation for the quadratic functional. The upper bound consists of two terms, one that mimics a classical bias-variance trade-off and a second that causes the typical elbow effect in quadratic functional estimation. Using a minimax optimal estimator of the quadratic functional as a test statistic, we derive an upper bound for the nonasymptotic minimax radius of testing for nonparametric alternatives. Interestingly, the term causing the elbow effect in the estimation case vanishes in the radius of testing. We provide a matching lower bound for the testing problem. By showing that any lower bound for the testing problem also yields a lower bound for the quadratic functional estimation problem, we obtain a lower bound for the risk of estimation. Lastly, we prove a matching lower bound for the term causing the elbow effect in the estimation problem. The results are illustrated considering Sobolev spaces and ordinary or super smooth error densities.

==> packages.tex <==
% 
\usepackage[english]{babel}
\RequirePackage{ucs}
\RequirePackage[utf8x]{inputenc}
%
% zeige labels am rand an.
% \usepackage[notref,notcite]{showkeys} 
%  aendere Anzeige der labels         
% \renewcommand{\showkeyslabelformat}[1]{%
%	\mbox{\dg \normalfont\tiny\ttfamily#1}}
%%
%
%\usepackage{lmodern} % font: Latin Modern
%\usepackage[right = 2cm, top=2.5cm, bottom=2.5cm,left=2cm]{geometry}
%
%
%
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{thmtools}
\usepackage{mathtools}
\usepackage{amsfonts}
%
%==========================================
\RequirePackage{amsthm,amsmath}
\RequirePackage{amssymb,amstext}
\RequirePackage{amsfonts,stmaryrd}
\RequirePackage{amsbsy} 
\RequirePackage{mathrsfs}
\RequirePackage{bm}
\RequirePackage{bbm}
\RequirePackage{aliascnt,ifthen}
\RequirePackage{graphicx}
\RequirePackage{color,calc}
%\RequirePackage{times}
\RequirePackage{url}
\RequirePackage{verbatim}

\RequirePackage{relsize}

\usepackage[pdfpagemode=UseOutlines ,plainpages=false,
%hypertexnames=false ,pdfpagelabels=TRUE ,
hyperindex=true,colorlinks=true]{hyperref}
	\makeatletter
	\Hy@breaklinkstrue
	\makeatother

\definecolor{darkred}{rgb}{0.6,0,0.1}
\definecolor{darkgreen}{rgb}{0,0.5,0}
\definecolor{darkblue}{rgb}{0,0,0.5}

\hypersetup{colorlinks ,linkcolor=gray ,filecolor=darkgreen,  urlcolor=blue ,citecolor=black}

\RequirePackage{paralist}

% BIBLIOGRAPHY
\usepackage{natbib}
\usepackage{hypernat}
\renewcommand{\cite}{\citet}
\bibliographystyle{abbrvnat}

%==========================================
% Packages Sandra
%==========================================
\usepackage{enumitem} % advanced enumeration
\usepackage{graphicx} % for including graphics
\usepackage{dsfont} % indicator function \mathds{1}
\usepackage{tikz} % tikz pgf: advanced drawing
\usetikzlibrary{shapes.geometric, arrows.meta, calc, positioning, shapes.multipart}
\usepackage[framemethod=TikZ]{mdframed}
\usepackage{ifthen}
\usepackage{supertabular} % tables with pagebreaks
\usepackage{booktabs}  % nicer tables
\usepackage{cases}
\usepackage{xcolor}
\usepackage{blindtext}
\usepackage{multirow}

\usepackage{cleveref}
\crefname{definition}{\color{\colde}Definition}{\color{\colde}Definitions}
\crefname{lemma}{\color{\colre}Lemma}{\color{\colre}Lemmata}
\crefname{proposition}{\color{\colre}Proposition}{\color{\colre}Propositions}
\crefname{requisite}{\color{\colrem}Requisite}{\color{\colrem}Requisites}
\crefname{theorem}{\color{\colre}Theorem}{\color{\colre}Theorems}
\crefname{corollary}{\color{\colre}Corollary}{\color{\colre}Corollaries}
\crefname{remark}{\color{\colrem}Remark}{\color{\colrem}Remarks}
\crefname{assumption}{\color{\colrem}Assumption}{\color{\colrem}Assumptions}
\crefname{illustration}{\color{\colil}Illustration}{\color{\colil}Illustrations}
\crefname{section}{\color{\colre}Section}{\color{\colre}Sections}
\crefname{appendix}{\color{\colre}Appendix}{\color{\colre}Appendices}
\numberwithin{equation}{section} 


